Mol-LLM: Multimodal Generalist Molecular LLM with Improved Graph Utilization

Recent advances in large language models (LLMs) have led to models that tackle diverse molecular tasks, such as chemical reaction prediction and molecular property prediction. Large-scale molecular instruction-tuning datasets have enabled sequence-only (e.g., SMILES or SELFIES) generalist molecular LLMs, and researchers are now exploring multimodal approaches that incorporate molecular structural information for further gains. However, a genuinely multimodal, generalist LLM that covers a broad spectrum of molecular tasks has yet to be fully investigated. We observe that naive next token prediction training ignores graph-structural information, limiting an LLM's ability to exploit molecular graphs. To address this, we propose (i) Molecular structure Preference Optimization (MolPO), which facilitates graph usage by optimizing preferences between pairs of correct and perturbed molecular structures, and (ii) an advanced graph encoder with a tailored pre-training strategy to improve the effect of graph utilization by MolPO. Building on these contributions, we introduce Mol-LLM, the first multimodal generalist model that (a) handles a broad spectrum of molecular tasks among molecular LLMs, (b) explicitly leverages molecular-structure information, and (c) takes advantage of extensive instruction tuning. Mol-LLM attains state-of-the-art or comparable results across the most comprehensive molecular-LLM benchmark-even on out-of-distribution datasets for reaction and property prediction, where it surpasses prior generalist molecular LLMs by a large margin.

==> NeurIPS2025/figure_tex/fig_gnn_downstream_ablation.tex <==
\begin{figure}[t]
  \centering
  %--- 첫 번째 ---
  \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\linewidth]{figures/val_qm9_homo_mae_tunegnn.pdf}
    % \caption{(a)}
  \end{subfigure}\hfill
  %--- 두 번째 ---
  \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\linewidth]{figures/val_forward_reaction_prediction_exact_match_ratio_tunegnn.pdf}
    % \caption{(b)}
  \end{subfigure}\hfill
  %--- 세 번째 ---
  \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\linewidth]{figures/val_reagent_prediction_exact_match_ratio_tunegnn.pdf}
    % \caption{(c)}
  \end{subfigure}\hfill
  % %--- 네 번째 ---
  % \begin{subfigure}[b]{0.24\textwidth}
  %   \includegraphics[width=\linewidth]{figures/HOMO_val_qm9_homo_avg_loss.pdf}
  %   \caption{(d)}
  % \end{subfigure}
% 서로 다른 GNN 구조와 사전학습 모델 파라미터 사용한 초기화에 따른 세 가지 downstream task 학습 성능 비교. Graph의 성능만을 비교하기 위해 1D sequence (SELFIES) 입력을 제외하고 task instruction과 2D 그래프만을 입력으로 사용했다.
  \caption{Learning curves for three downstream tasks, each initialized with different GNN architectures and their corresponding pre-trained weights. To isolate the effect of graph representations, we fed the model only the task instructions and 2D graphs, omitting the 1D SELFIES sequences.}
  \label{fig:gnn_ablation}
\end{figure}

==> NeurIPS2025/figure_tex/fig_gnn_pretraining.tex <==
\begin{figure}\centering
    \includegraphics[width=.9\textwidth]{figures/gnn_pretraining_task.pdf}
    \caption{(GNN pretraining)}
    \label{fig:gnn_pretraining}
    % \vspace{-0.5cm}
\end{figure}

==> NeurIPS2025/figure_tex/fig_preference_accuracy.tex <==
\begin{figure}[!t]\centering
    \includegraphics[width=.35\textwidth]{figures/fig3_preference_accuracy.png}
    \caption{Preference accuracy between chosen and rejected pairs on reaction prediction tasks (FS, RS, RP), with and without MolPO training.
    \fix{To be substituted with all In task + OOD task version}
    }
    \label{fig:preference_accuracy}
\end{figure}

==> NeurIPS2025/table_tex/tab_res_ablation_subtasks.tex <==



\begin{table}[h!]
\footnotesize
\centering
\caption{
Ablation study on the subtasks of Mol-LLM training datasets for investigation of multimodal balanced training of MolPO. First trained by SFT with 1D molecular sequence at three epochs as pretraining, and then additionally trained with two epochs for SFT with 1D molecular sequence, SFT with 1D and 2D, and MolPO, each.
}
\resizebox{\columnwidth}{!}{ % Resizes the table to fit the column width
\begin{tabular}{@{}lrrrrrrrrrrrr@{}}
\toprule
 &
  \multicolumn{1}{c}{FS} &
  \multicolumn{1}{c}{RS} &
  \multicolumn{1}{c}{RP} &
  \multicolumn{1}{c}{HOMO} &
  \multicolumn{1}{c}{ESOL} &
  \multicolumn{1}{c}{Lipo} &
  \multicolumn{1}{c}{Clintox} &
  \multicolumn{1}{c}{BACE} &
  \multicolumn{1}{c}{HIV} &
  \multicolumn{1}{c}{BBBP} &
  \multicolumn{1}{c}{Sider} &
  \multicolumn{1}{c}{\# Best} \\ \midrule
SFT S &
  0.672 &
  0.523 &
  0.177 &
  0.0041 &
  \textbf{1.12} &
  1.02 &
  \textbf{0.900} &
  0.814 &
  0.746 &
  0.863 &
  0.777 &
  2 \\
SFT S+G &
  0.652 &
  0.526 &
  0.184 &
  \textbf{0.0040} &
  1.13 &
  1.02 &
  0.879 &
  0.843 &
  0.736 &
  \textbf{0.896} &
  \textbf{0.780} &
  3 \\
MolPO &
  \textbf{0.678} &
  \textbf{0.537} &
  \textbf{0.199} &
  0.0041 &
  1.17 &
  \textbf{0.97} &
  0.868 &
  \textbf{0.845} &
  \textbf{0.756} &
  0.882 &
  0.770 &
  6 \\ \bottomrule
\end{tabular}%
}
\label{tab:combined_performance_metrics}
\end{table}


==> NeurIPS2025/table_tex/tab_res_ood_datasets.tex <==
\begin{table}[h!]
  \centering
  \footnotesize
  \caption{(a) Evaluation of O.O.D generalization on predicting water solubility (LogS) with RMSE on AQSOL dataset, and (b) reaction-prediction on Orderly dataset, which is non-USPTO.}
  \label{tab:general_results}

  \resizebox{\columnwidth}{!}{
  \begin{tabular}{@{}cc@{}}
    % ---------- AQSOL -------------------------------------------------
    \begin{subtable}[t]{0.5\columnwidth}
      \centering
      \label{tab:general_regression_alchemy_aqsol}
      \caption{}
      \begin{tabular}{@{}lr@{}}
        \toprule
        Model                                 & \multicolumn{1}{l}{LogS}  \\ \midrule
        % {\ul \textit{Semi-Generalist Models}} &                             \\
        {\ul \textit{Generalist Models}}      &                            \\
        LlaSMol                               & 1.32                       \\
        3D-MoLM                               & 2.72                       \\
        Mol-LLM (w/o GRAPH)                   & 1.10                       \\
        %Mol-LLM (w/o MolPO)                   & 1.02                       \\
        Mol-LLM                               & \textbf{1.02}              \\ \bottomrule
      \end{tabular}%
    \end{subtable}
    &
    % ---------- Orderly ------------------------------------------------
    \begin{subtable}[t]{0.9\columnwidth}
      \centering
      \label{tab:general_reaction_orderly}
        \caption{}
        \begin{tabular}{@{}llrrrr@{}}
        \toprule
        Task & Model & \multicolumn{1}{l}{EXACT (↑)} & \multicolumn{1}{l}{BLEU (↑)} & \multicolumn{1}{l}{MACCS FTS (↑)} & \multicolumn{1}{l}{VALIDITY (↑)} \\ \midrule
        \multirow{5}{*}{FS} & {\ul \textit{Semi-Generalist Models}} &                &       &       &       \\
                            & BioT5$^{*}$ (Reg.\ \& React.)         & 0.095          & 0.684 & 0.628 & 1.00  \\ \cmidrule(l){2-6} 
                            & \multicolumn{5}{l}{\textit{Generalist Models}}                                 \\
                            & LlaSMol$^{*}$                         & 0.350          & 0.754 & 0.881 & 1.00 \\
                            & Mol-LLM (w/o Graph)                        & 0.394 &    \textbf{0.814}   &   \textbf{0.900}    & 1.00  \\
                            %& Mol-LLM (w/o MolPO)                        & 0.394  &   0.800    &  0.878     & 1.00  \\
                            & Mol-LLM                        & \textbf{0.401} &     0.791  &    0.877   & 1.00  \\ \midrule
        \multirow{5}{*}{RS} & {\ul \textit{Semi-Generalist Models}} &                &       &       &       \\
                            & BioT5$^{*}$ (Reg.\ \& React.)         & 0.139          & 0.673 & 0.678 & 1.00  \\ \cmidrule(l){2-6} 
                            & {\ul \textit{Generalist Models}}      &                &       &       &       \\
                            & LlaSMol$^{*}$                         & 0.473          & 0.822 & 0.875 & 1.00 \\
                            & Mol-LLM (w/o Graph)                        & 0.727 &    0.920   &   0.936    & 1.00  \\
                            %& Mol-LLM (w/o MolPO)                        & 0.730  &   0.923    &  0.940     & 1.00  \\
                            & Mol-LLM                        & \textbf{0.738} &     \textbf{0.925}  &  \textbf{0.939}     & 1.00  \\ \bottomrule
        \end{tabular}%
    \end{subtable}
  \end{tabular}}
\end{table}
% \begin{table}[h!]
% \footnotesize\centering\setlength{\tabcolsep}{4.4pt}
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{cc}
% \begin{minipage}{0.5\textwidth}
% \centering
% \caption{RMSE performance comparison on AQSOL dataset for O.O.D data generalization in water solubility prediction.}
% \begin{tabular}{@{}l|c@{}}
% \toprule
% Model & AQSOL ($\downarrow$) \\ \midrule
% {\ul \textit{Semi-Generalist Models}} &  \\
% LlaSMol & 1.32 \\ \midrule
% \textit{\underline{Generalist Models}} &  \\
% Mol-LLM (Ours) & 1.01 \\ \bottomrule
% \end{tabular}%
% \label{tab:general_regression_alchemy_aqsol}
% \end{minipage} &

% \begin{minipage}{0.5\textwidth}
% \centering
% \caption{Performance comparison on reaction prediction task on Orderly dataset. 
% Each metric represents Exact match, MACCS FTS, molecule validity.}
% \begin{tabular}{@{}llrrrr@{}}
% \toprule
% Task & Model & \multicolumn{1}{l}{EXACT ($\uparrow$)} & \multicolumn{1}{l}{BLEU ($\uparrow$)} & \multicolumn{1}{l}{FTS ($\uparrow$)} & \multicolumn{1}{l}{VAL. ($\uparrow$)} \\ \midrule
% \multirow{5}{*}{FS} & {\ul \textit{Semi-Generalist Models}} & & & &  \\ 
% & BioT5+$^*$(Reg. \& React.) & 0.095 & 0.684 & 0.628 & 1.00 \\ \cmidrule(l){2-6} 
% & {\ul \textit{Generalist Models}} & & & &  \\ 
% & LlaSMol$^*$ & 0.350 & 0.754 & 0.881 & 0.997 \\ 
% & Mol-LLM (Ours) & 0.401 & & & 1.00 \\ \midrule
% \multirow{5}{*}{RS} & {\ul \textit{Semi-Generalist Models}} & & & &  \\ 
% & BioT5+$^*$(Reg. \& React.) & 0.139 & 0.673 & 0.678 & 1.00 \\ \cmidrule(l){2-6} 
% & {\ul \textit{Generalist Models}} & & & &  \\ 
% & LlaSMol$^*$ & 0.473 & 0.822 & 0.875 & 0.997 \\ 
% & Mol-LLM (Ours) & 0.738 & & & 1.00 \\ \bottomrule
% \end{tabular}%
% \label{tab:general_reaction_orderly}
% \end{minipage}
% \end{tabular}
% }
% \end{table}



% Generalization - Regression - alchemy Table
%\begin{table}[t!]
%\footnotesize\centering\setlength{\tabcolsep}{4.4pt}
%\caption{
%RMSE Performance comparison on AQSOL~\cite{} dataset for O.O.D data generalization in water solubility prediction.
%}
%\resizebox{0.5\textwidth}{!}{
%\begin{tabular}{@{}l|c@{}}
%\toprule
%Model & AQSOL ($\downarrow$) \\ \midrule
%{\ul \textit{Semi-Generalist Models}} &  \\
%LlaSMol                           & 1.32 \\ \midrule
%\textit{\underlineGeneralist Models}  &  \\
%Mol-LLM Resume (Ours)                               & 1.01 \\ \bottomrule
%\end{tabular}%
%}
%\label{tab:general_regression_alchemy_aqsol}
%\end{table}

% Generalization - Regression - alchemy Table
%\begin{table}[t!]
%\footnotesize\centering\setlength{\tabcolsep}{4.4pt}
%\caption{
%Performance comparison on molecule property tasks on Alchemy~\cite{} and AQSOL~cite{} dataset. MAE for Homo, Lumo, Gap tasks. * denotes performance evaluated based on the official checkpoint, bold denotes the best performance overall, and underline denotes the best performance of the generalist.
%}
%\resizebox{0.5\textwidth}{!}{
%\begin{tabular}{@{}l|cccc@{}}
%\toprule
%Model & Homo ($\downarrow$) & Lumo ($\downarrow$) & $\Delta \epsilon$($\downarrow$) & AQSOL ($\downarrow$) \\ \midrule
%{\ul \textit{Semi-Generalist Models}} &        &        &        &  \\
%BioT5+$^*$                            & 0.0143 & 0.0200 & 0.0289 &  \\ \midrule
%\textit{\underlineGeneralist Models}  &        &        &        &  \\
%Mol-LLM                               &        &        &        &  \\ \bottomrule
%\end{tabular}%
%}
%\label{tab:general_regression_alchemy_aqsol}
%\end{table}

==> NeurIPS2025/table_tex/tab_res_ood_reaction_orderly.tex <==
% Generalization - Reaction - Orderly Table
\begin{table}[t!]
\footnotesize\centering\setlength{\tabcolsep}{4.4pt}
\caption{
Performance comparison on reaction prediction task on ORDerly~\cite{Wigh2024ORDerlyDS} dataset.
FS, RS each represent Forward synthesis and Retrosynthesis.
}
\resizebox{\textwidth}{!} {
\begin{tabular}{@{}llcccccc@{}}
\toprule
Task & Model & EXACT ($\uparrow$) & BLEU ($\uparrow$) & RDK FTS ($\uparrow$) & MACCS FTS ($\uparrow$) & MORGAN FTS ($\uparrow$) & VALIDITY ($\uparrow$) \\ \midrule
\multirow{10}{*}{FS} & {\ul \textit{Semi-Generalist Models}} &       &       &       &       &       &      \\
                     & BioT5+$^*$(Reg. \& React.)            & 0.095 & 0.684 & 0.466 & 0.628 & 0.440 & 1.00 \\ \cmidrule(l){2-8} 
                     & {\ul \textit{Generalist Models}}      &       &       &       &       &       &      \\
                     & GPT-4                                 & 0.000 & -     & -     & 0.723 & -     & 0.87 \\
                     & Galactica$^*$                         & 0.000 & 0.156 & 0.180 & 0.322 & 0.118 & 0.49 \\
                     & 3D-MoLM$^*$                           & 0.000 & 0.157 & 0.101 & 0.288 & 0.114 & 0.01 \\
                     & ChemDFM$^*$                           & 0.000 & 0.253 & 0.294 & 0.428 & 0.250 & 0.04 \\
                     & LlaSMol$^*$                           & 0.350 & 0.754 & 0.762 & 0.881 & 0.744 & 1.00 \\
                     & Mol-LLM (w/o Graph)                   & 0.394 & 0.814     & 0.813     & 0.900 & 0.795     & 1.00 \\
                     & Mol-LLM                               & 0.401 & 0.791     & 0.758     & 0.877 & 0.740     & 1.00 \\ \midrule
\multirow{10}{*}{RS} & {\ul \textit{Semi-Generalist Models}} &       &       &       &       &       &      \\
                     & BioT5+$^*$(Reg. \& React.)            & 0.139 & 0.673 & 0.544 & 0.678 & 0.490 & 1.00 \\ \cmidrule(l){2-8} 
                     & {\ul \textit{Generalist Models}}      &       &       &       &       &       &      \\
                     & GPT-4                                 & 0.000 & -     & -     & 0.672 & -     & 0.65 \\
                     & Galactica$^*$                         & 0.000 & 0.250 & 0.297 & 0.398 & 0.227 & 0.38 \\
                     & 3D-MoLM$^*$                           & 0.000 & 0.155 & 0.287 & 0.396 & 0.165 & 0.01 \\
                     & ChemDFM$^*$                           & 0.000 & 0.239 & 0.285 & 0.406 & 0.244 & 0.05 \\
                     & LlaSMol$^*$                           & 0.473 & 0.822 & 0.842 & 0.875 & 0.808 & 0.99 \\
                     & Mol-LLM (w/o Graph)                   & 0.727 & 0.920     & 0.889     & 0.936 & 0.878     & 1.00 \\
                     & Mol-LLM                               & 0.738 & 0.925     & 0.897     & 0.939 & 0.886     & 1.00 \\ \bottomrule
\end{tabular}%
}
\label{tab:general_reaction_orderly}
\end{table}

==> NeurIPS2025/table_tex/tab_res_ood_reaction_presto.tex <==
% Generalization - Reaction - Presto Table
\begin{table}[t!]
\footnotesize\centering\setlength{\tabcolsep}{4.4pt}
\caption{
Performance comparison on reaction prediction task on Presto~\cite{} dataset.
FS, RS each represent Forward synthesis and Retrosynthesis.
* denotes performance evaluated based on the official checkpoint, bold denotes the best performance overall, and %underline denotes the best performance of the generalist.
}
\resizebox{\textwidth}{!} {
\begin{tabular}{@{}ll|l|cccccccc@{
\toprule 
& & MODEL & EXACT ($\uparrow$) & BLEU ($\uparrow$) & RDK FTS ($\uparrow$) & MACCS FTS ($\uparrow$) & MORGAN FTS %($\uparrow$) & VALIDITY ($\uparrow$) \\
\midrule

& \multirow{5}{*}{\centering \raisebox{-0.5ex} {\rotatebox{90}{FS }
& \textit{Semi-Generalist Models} \\[.2em]
& & $\text{BioT5+}^*$ & 0.130 & 0.635 & 0.443 & 0.558 & 0.417 & 1.00 \\
& & \textit{Generalist Models} \\[.2em]
& & $\text{LlaSMol}^*$ & 0.562 & 0.790 & 0.803 & 0.882 & 0.792 & 0.98 \\
& & Mol-LLM &  0.654 & 0.893 & 0.861 & %0.911 & 0.835 & {1.00} \\
\midrule

& \multirow{5}{*}{\centering \raisebox{-0.5ex} {\rotatebox{90}{RS }
& \textit{Semi-Generalist Models} \\[.2em]
& & $\text{BioT5+}^*$ & 0.127 & 0.636 & 0.440 & 0.556 & 0.416 & 1.00 \\
& & \textit{Generalist Models} \\[.2em]
& & $\text{LlaSMol}^*$ & 0.490 & 0.750 & 0.78}` & 0.855 & %0.759 & 0.97 \\
& &  Mol-LLM & 0.410 & 0.795 & 0.771 & 0.844 & 0.728 & 1.00 \\

\bottomrule


\end{tabular}
}
\label{tab:general_reaction_presto}
\end{table}

==> NeurIPS2025/table_tex/tab_res_reaction_forward.tex <==
% Full Reaction Prediction Table - Forward Synthesis
\begin{table}[t!]
\footnotesize\centering\setlength{\tabcolsep}{4.4pt}
\caption{
Performance comparison for forward synthesis task on Mol-Instructions~\cite{Fang2023MolInstructionsAL} and SMolInstruct \cite{Yu2024LlaSMolAL} datasets.
}
\resizebox{\columnwidth}{!} {
\begin{tabular}{@{}llcccccc@{}}
\toprule
Dataset & Model       & EXACT ($\uparrow$) & BLEU ($\uparrow$) & RDK FTS ($\uparrow$) & MACCS FTS ($\uparrow$) & MORGAN FTS ($\uparrow$) & VALIDITY ($\uparrow$) \\ \midrule
\multirow{15}{*}{Mol-Instructions} & {\ul \textit{Specialist Models}}      &       &       &       &       &       &      \\
                                   & InstructMol                           & 0.536 & 0.967 & 0.776 & 0.878 & 0.741 & 1.00 \\
                                   & MolCA$^*$                             & 0.000 & 0.321 & 0.329 & 0.494 & 0.253 & 0.01 \\ \cmidrule(l){2-8} 
                                   & {\ul \textit{Semi-Generalist Models}} &       &       &       &       &       &      \\
                                   & Mol-Instructions$^*$                  & 0.052 & 0.302 & 0.232 & 0.291 & 0.197 & 1.00 \\
                                   & BioT5+$^*$(Cls. \& Trans.)            & 0.000 & 0.206 & 0.081 & 0.152 & 0.069 & 0.98 \\
                                   & BioT5+$^*$(Reg. \& React.)            & 0.864 & 0.993 & 0.949 & 0.975 & 0.935 & 1.00 \\ \cmidrule(l){2-8} 
                                   & {\ul \textit{Generalist Models}}      &       &       &       &       &       &      \\
                                   & GPT-4 (5-shot)                        & 0.021 & 0.580 & 0.627 & 0.728 & 0.557 & 0.93 \\
                                   & Galactica                             & 0.000 & 0.468 & 0.156 & 0.257 & 0.097 & 0.95 \\
                                   & 3D-MoLM$^*$                           & 0.000 & 0.081 & 0.223 & 0.391 & 0.098 & 0.01 \\
                                   & ChemDFM$^*$                           & 0.000 & 0.028 & 0.104 & 0.142 & 0.077 & 0.07 \\
                                   & LlaSMol$^*$                           & 0.743 & 0.835 & 0.920 & 0.955 & 0.910 & 0.95 \\
                                   & Mol-LLM (w/o Graph)                   & 0.893 & 0.963 & 0.968 & 0.983 & 0.960 & 1.00 \\
        & Mol-LLM     & \textbf{0.911}     & \textbf{0.969}    & \textbf{0.976}       & \textbf{0.987}         & \textbf{0.967}          & 1.00                  \\ \midrule
\multirow{14}{*}{SMolInstruct}     & {\ul \textit{Specialist Models}}      &       &       &       &       &       &      \\
                                   & MolCA$^*$                             & 0.000 & 0.209 & 0.252 & 0.357 & 0.196 & 0.01 \\ \cmidrule(l){2-8} 
                                   & {\ul \textit{Semi-Generalist Models}} &       &       &       &       &       &      \\
                                   & Mol-Instructions$^*$                  & 0.003 & 0.149 & 0.139 & 0.184 & 0.111 & 1.00 \\
                                   & BioT5+$^*$(Cls. \& Trans.)            & 0.000 & 0.286 & 0.107 & 0.187 & 0.089 & 0.97 \\
                                   & BioT5+$^*$(Reg. \& React.)            & 0.081 & 0.455 & 0.418 & 0.537 & 0.376 & 1.00 \\ \cmidrule(l){2-8} 
                                   & {\ul \textit{Generalist Models}}      &       &       &       &       &       &      \\
                                   & GPT-4 (5-shot)                        & 0.011 & 0.451 & 0.520 & 0.634 & 0.440 & 0.87 \\
                                   & Galactica$^*$                         & 0.000 & 0.241 & 0.292 & 0.377 & 0.202 & 0.36 \\
                                   & 3D-MoLM$^*$                           & 0.000 & 0.086 & 0.226 & 0.296 & 0.117 & 0.01 \\
                                   & ChemDFM$^*$                           & 0.002 & 0.046 & 0.125 & 0.178 & 0.109 & 0.08 \\
        & LlaSMol$^*$ & \textbf{0.629}     & \textbf{0.883}    & \textbf{0.871}       & \textbf{0.919}         & \textbf{0.848}          & 0.99                  \\
                                   & Mol-LLM (w/o Graph)                   & 0.584 & 0.867 & 0.847 & 0.904 & 0.815 & 1.00 \\
                                   & Mol-LLM                               & 0.601 & 0.873 & 0.853 & 0.908 & 0.823 & 1.00 \\ \bottomrule
\end{tabular}%
}
\label{tab:reaction_prediction_forward}
\end{table}

==> NeurIPS2025/table_tex/tab_res_reaction_reagent.tex <==
% Full Reaction Prediction Table - Reagent Prediction
\begin{table}[t!]
\footnotesize\centering\setlength{\tabcolsep}{4.4pt}
\caption{
Performance comparison for reagent prediction task on Mol-Instructions~\cite{Fang2023MolInstructionsAL} dataset.
}
\resizebox{\columnwidth}{!} {
\begin{tabular}{@{}lcccccc@{}}
\toprule
Model   & EXACT ($\uparrow$) & BLEU ($\uparrow$) & RDK FTS ($\uparrow$) & MACCS FTS ($\uparrow$) & MORGAN FTS ($\uparrow$) & VALIDITY ($\uparrow$) \\ \midrule
{\ul \textit{Specialist Models}}      &       &       &       &       &       &      \\
InstructMol                           & 0.129 & 0.610 & 0.444 & 0.539 & 0.400 & 1.00 \\
MolCA$^*$                             & 0.000 & 0.002 & 0.033 & 0.115 & 0.012 & 0.01 \\ \midrule
{\ul \textit{Semi-Generalist Models}} &       &       &       &       &       &      \\
Mol-Instructions                      & 0.044 & 0.224 & 0.237 & 0.364 & 0.213 & 1.00 \\
BioT5+$^*$(Cls. \& Trans.)            & 0.000 & 0.169 & 0.038 & 0.056 & 0.015 & 0.96 \\
BioT5+$^*$(Reg. \& React.)            & 0.257 & 0.695 & 0.539 & 0.621 & 0.512 & 1.00 \\ \midrule
{\ul \textit{Generalist Models}}      &       &       &       &       &       &      \\
GPT-4 (5-shot)                        & 0.000 & 0.133 & 0.077 & 0.228 & 0.071 & 0.72 \\
Galactica                             & 0.000 & 0.141 & 0.036 & 0.127 & 0.051 & 0.99 \\
3D-MoLM$^*$                           & 0.000 & 0.042 & 0.039 & 0.218 & 0.077 & 0.01 \\
ChemDFM$^*$                           & 0.000 & 0.014 & 0.033 & 0.099 & 0.027 & 0.06 \\
LlaSMol$^{*}$                         & 0.000 & 0.050 & 0.041 & 0.199 & 0.050 & 0.93 \\
Mol-LLM (w/o Graph)                   & 0.202 & 0.557 & 0.497 & 0.586 & 0.461 & 1.00 \\
Mol-LLM & \textbf{0.225}     & \textbf{0.578}    & \textbf{0.517}       & \textbf{0.600}         & \textbf{0.485}          & 1.00                  \\ \bottomrule
\end{tabular}%
}
\label{tab:reaction_prediction_reagent}
\end{table}

==> NeurIPS2025/table_tex/tab_res_reaction_retrosynthesis.tex <==
% Full Reaction Prediction Table - Retrosynthesis
\begin{table}[t!]
\footnotesize\centering\setlength{\tabcolsep}{4.4pt}
\caption{
Performance comparison for retrosynthesis task on Mol-Instructions~\cite{Fang2023MolInstructionsAL} and SMolInstruct \cite{Yu2024LlaSMolAL} datasets.
}
\resizebox{\columnwidth}{!} {
\begin{tabular}{@{}llcccccc@{}}
\toprule
Dataset & Model & EXACT ($\uparrow$) & BLEU ($\uparrow$) & RDK FTS ($\uparrow$) & MACCS FTS ($\uparrow$) & MORGAN FTS ($\uparrow$) & VALIDITY ($\uparrow$) \\ \midrule
\multirow{15}{*}{Mol-Instructions} & {\ul \textit{Specialist Models}}      &                &                &                &                &                &      \\
                                   & InstructMol                           & 0.407          & 0.941          & 0.753          & 0.852          & 0.714          & 1.00 \\
                                   & MolCA$^*$                             & 0.000          & 0.652          & 0.936          & 0.880          & 0.722          & 0.01 \\ \cmidrule(l){2-8} 
                                   & {\ul \textit{Semi-Generalist Models}} &                &                &                &                &                &      \\
                                   & Mol-Instructions$^*$                  & 0.069          & 0.407          & 0.303          & 0.359          & 0.268          & 1.00 \\
                                   & BioT5+$^*$(Cls. \& Trans.)            & 0.001          & 0.095          & 0.114          & 0.195          & 0.104          & 0.97 \\
                                   & BioT5+$^*$(Reg. \& React.)            & 0.642          & 0.969          & 0.897          & 0.930          & 0.866          & 1.00 \\ \cmidrule(l){2-8} 
                                   & {\ul \textit{Generalist Models}}      &                &                &                &                &                &      \\
                                   & GPT-4 (5-shot)                        & 0.012          & 0.573          & 0.531          & 0.716          & 0.506          & 0.77 \\
                                   & Galactica                             & 0.000          & 0.452          & 0.167          & 0.274          & 0.134          & 0.99 \\
                                   & 3D-MoLM$^*$                           & 0.000          & 0.069          & 0.270          & 0.451          & 0.117          & 0.01 \\
                                   & ChemDFM$^*$                           & 0.000          & 0.224          & 0.360          & 0.440          & 0.234          & 0.03 \\
                                   & LlaSMol$^*$                           & 0.453          & 0.722          & 0.826          & 0.885          & 0.788          & 0.95 \\
                                   & Mol-LLM (w/o Graph)                   & 0.510          & 0.839          & 0.835          & 0.886          & 0.797          & 1.00 \\
                                   & Mol-LLM                               & \textbf{0.538} & \textbf{0.845} & \textbf{0.843} & \textbf{0.893} & \textbf{0.808} & 1.00 \\ \midrule
\multirow{14}{*}{SMolInstruct}     & {\ul \textit{Specialist Models}}      &                &                &                &                &                &      \\
                                   & MolCA$^*$                             & 0.000          & 0.503          & 0.716          & 0.760          & 0.589          & 0.01 \\ \cmidrule(l){2-8} 
                                   & {\ul \textit{Semi-Generalist Models}} &                &                &                &                &                &      \\
                                   & Mol-Instructions$^*$                  & 0.015          & 0.402          & 0.223          & 0.285          & 0.191          & 1.00 \\
                                   & BioT5+$^*$(Cls. \& Trans.)            & 0.000          & 0.085          & 0.095          & 0.170          & 0.085          & 0.97 \\
                                   & BioT5+$^*$(Reg. \& React.)            & 0.152          & 0.662          & 0.623          & 0.751          & 0.567          & 1.00 \\ \cmidrule(l){2-8} 
                                   & {\ul \textit{Generalist Models}}      &                &                &                &                &                &      \\
                                   & GPT-4 (5-shot)                        & 0.013          & 0.523          & 0.499          & 0.686          & 0.465          & 0.76 \\
                                   & Galactica$^*$                         & 0.000          & 0.346          & 0.341          & 0.447          & 0.272          & 0.43 \\
                                   & 3D-MoLM$^*$                           & 0.000          & 0.162          & 0.220          & 0.372          & 0.128          & 0.01 \\
                                   & ChemDFM$^*$                           & 0.000          & 0.257          & 0.304          & 0.443          & 0.252          & 0.03 \\
                                   & LlaSMol$^*$                           & 0.323          & 0.759          & 0.749          & 0.827          & 0.699          & 0.99 \\
                                   & Mol-LLM (w/o Graph)                   & 0.363          & 0.772          & 0.752          & 0.828          & 0.699          & 1.00 \\
                                   & Mol-LLM                               & \textbf{0.377} & \textbf{0.779} & \textbf{0.760} & \textbf{0.832} & \textbf{0.707} & 1.00 \\ \bottomrule
\end{tabular}%
}
\label{tab:reaction_prediction_retrosynthesis}
\end{table}

==> NeurIPS2025/table_tex/tab_training_data.tex <==
% Instruction dataset table
\begin{table}[t]
\footnotesize\centering\setlength{\tabcolsep}{4.4pt}
\caption{
Details of Mol-LLM instruction tuning training data and its sources.
}
% \resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcc@{}}
\toprule
TASKS                                  & \# Samples & DATA SOURCES \\ \midrule
Property Prediction (Regression)       & 1.4M       & MoleculeNet  \\
Property Prediction (Classification)   & 58K        & MoleculeNet  \\
Forward Reaction Prediction            & 1.1M       & USPTO        \\
Retrosynthesis                         & 1M         & USPTO 500MT  \\
Reagent Prediction                     & 120K       & USPTO 500K   \\ 
Molecule Captioning                    & 50K        & ChEBI-20     \\
Description-Guided Molecule Generation & 50K        & ChEBI-20     \\
Name Conversion                        & 600K       & PubChem      \\ \bottomrule
\end{tabular}%
% }
\label{tab:instruction_stat}
\vspace{-0.5cm}
\end{table}

==> NeurIPS2025/table_tex/tab_translation_plus_ood.tex <==
\begin{table}[t!]
  \centering
  \caption{(Left) Performance comparison for translation tasks on ChEBI-20~\cite{Edwards2022TranslationBM} and SMolInstruct \cite{Yu2024LlaSMolAL} datasets. (Right) Evaluation of OOD generalization for reaction prediction on the ORDerly dataset, which is non-USPTO, and water solubility (LogS) on the AqSol dataset.}
  \label{tab:combined}
  %------------ Translation ------------
  \begin{subtable}[t]{0.45\columnwidth}  % 폭은 전체의 45 %
    \centering
    % \caption{Performance comparison for translation tasks on ChEBI-20~\cite{Edwards2022TranslationBM} and SMolInstruct \cite{Yu2024LlaSMolAL} datasets.}
    \label{tab:A}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}lcccc@{}}
\toprule
Dataset                               & \multicolumn{4}{c}{ChEBI-20 / SMolInstruct}                                     \\ \midrule
Task                                  & \multicolumn{2}{c}{Molecule Generation}        & \multicolumn{2}{c}{Molecule Captioning}                          \\ \midrule
Model & EXACT ($\uparrow$) & MACCS FTS ($\uparrow$) & BLEU-4 ($\uparrow$) & METEOR ($\uparrow$) \\ \midrule
{\ul \textit{Specialist Models}}      &               &               &                        &                        \\
GIT-Mol                               & 0.051 / \ \ NA \ & 0.738 / \ \ NA \ & 0.263 / \ \ NA \  
     & 0.533 / \ \ NA \        \\
InstructMol                           & \ \ NA \ / \ \ NA \ & \ \ NA \ / \ \ NA \ & 0.371 / \ \ NA \ & 0.509 / \ \ NA \ \\
MolT5                                 & 0.311 / 0.317 & 0.834 / 0.879 & 0.508 / 0.366           & 0.614 / 0.515          \\
MolCA$^*$                             & \ \ NA \ / \ \ NA \ & \ \ NA \ / \ \ NA \ & 0.540 / 0.510 & 0.652 / 0.628          \\
MolXPT                                & 0.215 / \ \ NA \ & 0.859 / \ \ NA \ & 0.505 / \ \ NA \   
     & 0.626 / \ \ NA \         \\
Text+Chem T5                          & 0.322 / \ \ NA \ & 0.901 / \ \ NA \ & 0.542 / \ \ NA \   
     & 0.648 / \ \ NA \         \\ \midrule
{\ul \textit{Semi-Generalist Models}} &               &               &                        &                        \\
Mol-Instructions                      & 0.016 / 0.045 & 0.167 / 0.475 & 0.171 / 0.020          & 0.271 / 0.124          \\
BioT5+$^*$(Cls. \& Trans.)            & 0.557 / 0.519 & 0.907 / 0.897 & 0.591 / 0.582          & 0.680 / 0.677          \\
BioT5+$^*$(Reg. \& React.)            & 0.537 / 0.416 & 0.897 / 0.867 & 0.216 / 0.221          & 0.323 / 0.321          \\ \midrule
{\ul \textit{Generalist Models}}      &               &               &                        &                        \\
GPT-4 (5-shot)                        &\quad--\quad/ 0.040 &\quad--\quad/ 0.736 &\quad--\quad/\qquad--&\quad--\quad/\qquad-- \\
Galactica$^*$                         & 0.000 / 0.000 & 0.264 / 0.271 & 0.000 / 0.000          & 0.004 / 0.005          \\
3D-MoLM$^*$                           & 0.000 / 0.000 & 0.000 / 0.000 & 0.171 / 0.167          & 0.326 / 0.329          \\
ChemDFM$^*$                           & 0.018 / 0.041 & 0.165 / 0.297 & 0.031 / 0.035          & 0.078 / 0.085          \\
LlaSMol$^*$                           & 0.274 / 0.180 & 0.871 / 0.845 & 0.333 / 0.328          & 0.466 / 0.470          \\
Mol-LLM (w/o Graph)                   & 0.431 / 0.362 & 0.903/ \textbf{0.888}  & 0.482 / 0.477          & 0.587 / 0.585          \\
Mol-LLM                               & \textbf{0.443 / 0.368} & \textbf{0.906} / 0.887 & \textbf{0.493} / \textbf{0.482} & \textbf{0.599} / \textbf{0.589} \\ \bottomrule
\end{tabular}%
}
  \end{subtable}
  \hfill                    % 서브테이블 사이 간격
  %------------ OOD ------------
  \begin{subtable}[t]{0.54\linewidth}
    \centering
    % \caption{Evaluation of OOD generalization for reaction prediction on the ORDerly dataset, which is non-USPTO, and water solubility (LogS) on the AqSol dataset.}
    \label{tab:B}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}lccccc@{}}
\toprule
Dataset                               & AqSol & \multicolumn{4}{c}{ORDerly}            \\ \midrule
Task    & LogS                & \multicolumn{2}{c}{Forward Synthesis}       & \multicolumn{2}{c}{Retrosynthesis}          \\ \midrule
Model   & RMSE ($\downarrow$) & EXACT ($\uparrow$) & MACCS FTS ($\uparrow$) & EXACT ($\uparrow$) & MACCS FTS ($\uparrow$) \\ \midrule
{\ul \textit{Semi-Generalist Models}} &       &       &                &       &       \\
BioT5+$^*$(Reg. \& React.)            & 1.81  & 0.095 & 0.628          & 0.139 & 0.678 \\ \midrule
{\ul \textit{Generalist Models}}      &       &       &                &       &       \\
GPT-4                                 & -     & -     & -              & -     & -     \\
Galactica$^*$                         & 3.20  & 0.000 & 0.322          & 0.000 & 0.398 \\
3D-MoLM$^*$                           & 2.72  & 0.000 & 0.288          & 0.000 & 0.396 \\
ChemDFM$^*$                           & 6.98  & 0.017 & 0.428          & 0.000 & 0.406 \\
LlaSMol$^*$                           & 1.32  & 0.350 & 0.881          & 0.473 & 0.875 \\
Mol-LLM (w/o Graph)                   & 1.10  & 0.394 & \textbf{0.900} & 0.727 & 0.936 \\
Mol-LLM & \textbf{1.02}       & \textbf{0.401}     & 0.877                  & \textbf{0.738}     & \textbf{0.939}         \\ \bottomrule
\end{tabular}%
}
  \end{subtable}

\end{table}
